FormLM: Recommending Creation Ideas for Online Forms by Modelling Semantic and Structural Information

Online forms are widely used to collect data from human and have a multi-billion market. Many software products provide online services for creating semi-structured forms where questions and descriptions are organized by pre-defined structures. However, the design and creation process of forms is still tedious and requires expert knowledge. To assist form designers, in this work we present FormLM to model online forms (by enhancing pre-trained language model with form structural information) and recommend form creation ideas (including question / options recommendations and block type suggestion). For model training and evaluation, we collect the first public online form dataset with 62K online forms. Experiment results show that FormLM significantly outperforms general-purpose language models on all tasks, with an improvement by 4.71 on Question Recommendation and 10.6 on Block Type Suggestion in terms of ROUGE-1 and Macro-F1, respectively.

==> 3-Dataset.tex <==
\label{sec:dataset}

Since there is no existing dataset for online forms, we constructed our own form dataset by crawling public online forms created on a popular online form website. We filtered out forms with low quality (details in Appendix~\ref{appendix:dataset}) and only considered English forms in this work. We totally collected 62K public forms across different domains, \textit{e.g.}, education, finance, medical, community activities, etc., 
and split them into 50K for training, 6K for validation, and 6K for testing.

Due to the structured nature of online forms, we further parsed the crawled HTML pages into JSON format by extracting valid contents and associating each block with its type. %\footnote{Google Forms question type: \href{https://support.google.com/docs/answer/7322334}{https://support.google.com/docs/answer/7322334}}.
% Below is legacy ----------------

%Apart from question blocks, there are description blocks in the crawled Google forms which contain text, image, or video information. We associated these blocks with \textit{Description} type and only kept the text information because only around 0.1\% blocks contain video and 2.0\% blocks contain image.
\reffig{Fig.type} shows the distribution of block types in our collected dataset.
\begin{figure}[h]
    \centering 
    \includegraphics[width=1\columnwidth]{images/type.pdf}
    \caption{Distribution of block types in Online Form Dataset.}
    \label{Fig.type}
\end{figure}

More details of the dataset statistics and the data curation process are included in Appendix~\ref{appendix:dataset}.

%To support the evaluation of \textit{Forms Intents Analysis}, we \todo{introduce the data labelling process}. More details of the Public Forms Dataset statistics and quality control process are included in Appendix~\ref{appendix:dataset}.
